A Parallel Batch-Dynamic Data Structure for the Closest Pair Problem

We propose a theoretically-efficient and practical parallel batch-dynamic data structure for the closest pair problem. Our solution is based on a serial dynamic closest pair data structure by Golin et al., and supports batches of insertions and deletions in parallel. For a data set of size $n$, our data structure supports a batch of insertions or deletions of size $m$ in $O(m(1+\log ((n+m)/m)))$ expected work and $O(\log (n+m)\log^*(n+m))$ depth with high probability, and takes linear space. The key techniques for achieving these bounds are a new work-efficient parallel batch-dynamic binary heap, and careful management of the computation across sets of points to minimize work and depth. We provide an optimized multicore implementation of our data structure using dynamic hash tables, parallel heaps, and dynamic $k$-d trees. Our experiments on a variety of synthetic and real-world data sets show that it achieves a parallel speedup of up to 38.57x (15.10x on average) on 48 cores with hyper-threading. In addition, we also implement and compare four parallel algorithms for static closest pair problem, for which we are not aware of any existing practical implementations. On 48 cores with hyper-threading, the static algorithms achieve up to 51.45x (29.42x on average) speedup, and Rabin's algorithm performs the best on average. Comparing our dynamic algorithm to the fastest static algorithm, we find that it is advantageous to use the dynamic algorithm for batch sizes of up to 20\% of the data set. As far as we know, our work is the first to experimentally evaluate parallel closest pair algorithms, in both the static and the dynamic settings.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file


==> code/code-binaryheap-async.tex <==
\begin{algorithm}[t]
  \caption{The \async algorithm}\label{alg:heap-async}
  \SetAlgoLined
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \Input{A binary min-heap of size $n$ with $m$ updates to change key $k_i$ to $k'_i$ on node $n_i$.}
  \Output{An updated binary heap.} 

  \ForEach {\upshape $v$ in the heap} {
     $v$'s flag is $1$ if $v$'s key is increased, $0$ otherwise
  }
  \ForEach {\upshape $v$ with flag $1$} {
        \textsc{Down-Heap}($v$)
  }
  \ForEach {\upshape $v$ in the heap} {
     $v$'s flag is $1$ if $v$'s key is decreased, $0$ otherwise
  }
  Mark the wait-flag to 1 for nodes with both subtrees having increased keys\\
  \ForEach {\upshape $v$ with flag $1$} {
        \textsc{Up-Heap}($v$)
  }
  \SetKwProg{myproc}{Procedure}{}{}
  \myproc{\upshape \textsc{Down-Heap}($v$)} {
       \If {$v$ is leaf} {
          \If {\upshape CAS($v$.flag, $1$, $0$) is failed} {
              $v$.flag $\gets 0$\label{line:jump-down-leaf}\\
              \textsc{Down-Heap}($v$'s parent)
          }
      }
      Let $lC$ be $v$'s left child and $rC$ be right child\\
      \lIf {\upshape CAS($lC$.flag, $1$, $2$)} {Quit}
      \lIf {\upshape CAS($rC$.flag, $1$, $2$)} {Quit}
      Let $c$ be $lC$ or $rC$ with smaller key\\
      \If {\upshape $c$.key $<v$.key} {
          Swap $v$'s and $c$'s keys\\
          $c$'.flag $\gets 1$\\
          \lIf {\upshape CAS($v$.flag, $1$, $0$)} {
            \textsc{Down-Heap}($c$)
          } \Else {
            $v$.flag $\gets 0$\label{line:jump-down}\\
            Run \textsc{Down-Heap}($v$'s parent) and \textsc{Down-Heap}($c$) in parallel
          }
      } 
      \Else {
          \If {\upshape CAS($v$.flag, $1$, $0$) is failed} {
              $v$.flag $\gets 0$\label{line:jump-down2}\\
              \textsc{Down-Heap}($v$'s parent)
          }
      }
  }
  \myproc{\upshape \textsc{Up-Heap}($v$)} {
      \If {\upshape $v$ is root} { 
         \If {\upshape CAS($v$.flag, $1$, $0$) failed} {
              $v$.flag $\gets 0$\label{line:jump-up-root}\\
              \textsc{Up-Heap}($v$.leftchild)
          } 
          Quit
      }
      \lIf {\upshape CAS($v$.parent.wait-flag, 1, 0)} {Quit}
      \lIf {\upshape CAS($v$.parent.flag, 1, 2)} {Quit}
      \lIf {\upshape $v$.sibling has smaller key} {$v\gets v$.sibling}
      \lIf {\upshape $v$.key $<v$.parent.key} {
          Swap $v$'s and $v$.parent's keys
      }
      \lIf {\upshape CAS($v$.flag, $1$, $0$)} {
        \textsc{Up-Heap}($v$.parent)
      } \Else {
          $v$.flag $\gets 0$\label{line:jump-up}\\
          Run \textsc{Up-Heap}($v$.parent) and \textsc{Up-Heap}($v$.leftchild) in parallel
      }
  }  
\end{algorithm}


==> code/code-grid-insert.tex <==
\begin{algorithm}[t]
\SetAlgoLined
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \Input{$(S_i, S_i', p_i, q_i, d_i)$ and $H_i$ for $1\leq i \leq L$; a batch $Q$ to be inserted.}

 \SetKwFunction{algo}{algo}\SetKwFunction{proc}{proc}
 \SetKwProg{myalg}{Algorithm}{}{}
 \SetKwProg{myproc}{Procedure}{}{}

 \myalg{\textsc{Main}()}{
   \textsc{Insert}($Q$, $\emptyset$, $1$)\;\label{line:grid-insert:call}
 }{}
   
 \myproc{\textsc{Insert}($Q_{i}$, $\down_{i}$, $i$)}{\label{line:grid-insert:insert-proc}
   $(Q_{i+1}$, $\down_{i+1}) :=$ \textsc{GridInsert}$(Q_{i}$, $\down_{i}$, $i)$\;\label{line:grid-insert:grid}
   \textsc{HeapUpdate}$(i)$\;\label{line:grid-insert:heap}
   \lIf{$(Q_{i+1}\cup \down_{i+1}) \neq \emptyset$}{
     \textsc{Insert}($Q_{i+1}$, $\down_{i+1}$, $i+1$)
   }\label{line:grid-insert:recur-insert}
 }
 
 \myproc{\textsc{GridInsert}$(Q_{i}$, $\down_{i}$, $i)$}{
   Determine if $p_i$, $q_i$, and $d_i$ should change when inserting $Q_i$ and $down_i$, which happens with probability $(|Q_i|+|down_i|)/(|Q_i|+|down_i|+|S_i|)$, or if a new point is closer to $p_i$ than the previously closest point $q_i$. \label{line:grid-insert:pivot}

    If $p_i$, $q_i$, or $d_i$ change on Line~\ref{line:grid-insert:pivot}, or if $i>L$, call \textsc{Build}$(Q_{i}\cup \down_{i}\cup S_i, i)$ to build subsequent levels, and terminate the batch insertion.\label{line:grid-insert:rebuild}

   Insert each point in $\down_{i}$ and $Q_{i}$ into the dictionary of $S_i$ in parallel.\label{line:grid-insert:insert}

   For each point $x$ in $Q_{i}$ in parallel, check if it is sparse in $S_i$. If so, insert $x$ into the dictionary of $S_i'$, and otherwise, insert $x$ into $Q_{i+1}$.\label{line:grid-insert:check1}

   For each point $x$ in $\down_{i}$ in parallel, check if it is sparse in $S_i$. If so, insert $x$ into the dictionary of $S_i'$, and otherwise, insert $x$ into $\down_{i+1}$.\label{line:grid-insert:check2}

   In parallel, for each point $x$ in $Q_{i}$, and for each point $r$ in the neighborhood $N(x, S_i')$, delete $r$ from $S_i'$, and insert $r$ into $\down_{i+1}$.\label{line:grid-insert:check3}

   \Return $(Q_{i+1},\down_{i+1})$\;
 }

 \caption{Batch Insert}\label{alg:grid-insert}
\end{algorithm}


==> code/code-heap-pull-delete.tex <==
\begin{algorithm}[t]
\SetAlgoLined
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \Input{$(S_i, S_i', p_i, q_i, d_i)$ and $H_i$ for $1\leq i \leq L$; a batch $Q$ to be deleted.}

 \SetKwFunction{algo}{algo}\SetKwFunction{proc}{proc}
 \SetKwProg{myalg}{Algorithm}{}{}
 \SetKwProg{myproc}{Procedure}{}{}

 \myalg{\textsc{Main}()}{\label{line:heap-delete:main}
   \textsc{Delete}($\emptyset$, $1$)\;\label{line:heap-delete:call}
   Perform \textsc{HeapUpdate-Pull($i$)} for $1\leq i < k$ in parallel.\label{line:heap-delete:pull-call-last}
 }{}

 \myproc{\textsc{Delete}($\up_{i}$, $i$)}{\label{line:heap-delete:proc}
   $\up_{i-1}:=$ \textsc{GridDelete}($\up_{i}$, $i$)\;\label{line:heap-delete:grid-call}
   \Spawn \textsc{HeapUpdate-Pull}($i+k$)\;\label{line:heap-delete:pull-call}
   \Indp \textsc{Delete}($\up_{i-1}$, $i-1$)\;\label{line:heap-delete:grid-call-next}
   \Indm \Sync\label{line:heap-delete:sync}
 }

 \caption{Batch Delete with Parallel Heap Update}\label{alg:heap-delete}
\end{algorithm}


==> code/code-heap-pull-insert.tex <==
\begin{algorithm}[t]
\SetAlgoLined
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \Input{$(S_i, S_i', p_i, q_i, d_i)$ and $H_i$ for $1\leq i \leq L$; a batch $Q$ to be inserted; point set $M_1$ that start moving at level $i$ and point set $M_2$ that stop moving at level $i$.}

 \SetKwFunction{algo}{algo}\SetKwFunction{proc}{proc}
 \SetKwProg{myalg}{Algorithm}{}{}
 \SetKwProg{myproc}{Procedure}{}{}

 \myalg{\textsc{Main}()}{\label{line:heap-insert:main}
   \textsc{Insert}($Q$, $\emptyset$, $1$)\;\label{line:heap-insert:call}
 }{}
   
 \myproc{\textsc{Insert}($Q_{i}$, $\down_{i}$, $i$)}{\label{line:heap-insert:insert-proc}
   $(Q_{i+1}, \down_{i+1}) :=$ \textsc{GridInsert}($Q_{i}$, $\down_{i}$, $i$)\;\label{line:heap-insert:grid-call}
   \Spawn \textsc{HeapUpdate-Pull}($i$)\;\label{line:heap-insert:pull-call}
   \Indp \textsc{Insert}($Q_{i+1}$, $\down_{i+1}$, $i+1$)\;\label{line:heap-insert:next-grid-call}
   \Indm \Sync\label{line:heap-insert:sync}
 }
 
 \myproc{\textsc{HeapUpdate-Pull}($i$)}{\label{line:heap-insert:pull-proc}
    Batch delete $d_i^*(p)\ \forall p\in M_1$ from $H_i$.\label{line:heap-insert:del}
    
    Compute and batch insert $d^*_i(q)\ \forall q\in M_2$ into $H_i$.\label{line:heap-insert:ins}
    
    Batch delete $d_i^*(q)$ from $H_i$ if $d_i^*(q)=d(q,p)$ and $p$ started moving at initiator level $i-l$ where $0\leq l\leq k$.\label{line:heap-insert:start-update}

    Batch delete $d^*(q)$ from $H_i$ if $d(q,p)<d^*(q)$ and $p$ stopped moving at initiator level $i-l$ where $0\leq l\leq k$.\label{line:heap-insert:stop-update}

    Re-compute $d^*(q)$ for each $q$ deleted on Lines 11--12, and batch insert then into $H_i$.\label{line:heap-insert:recomp}
 }

 \caption{Batch Insert with Parallel Heap Updates}\label{alg:heap-insert}
\end{algorithm}


==> main/plots-all.tex <==
\begin{figure}[]
\centering
  \begin{minipage}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{plot/Thr-5D-Uniform-10M.pdf}
  \end{minipage} %
  \begin{minipage}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{plot/Thr-3D-Cosmo-298M.pdf}
  \end{minipage} %
  \caption{Plot of throughput vs.\ batch size in log-log scale for our parallel batch-dynamic algorithm on 5D-Uniform-10M and 3D-Cosmo-298M. The throughput is computed as the number of points processed per second.
  The algorithm run on 48-cores with hyper-threading and 1 thread has a suffix of "48h" and "1t", respectively.
For 3D-Cosmo-298M, we omit the 1-thread time for dynamic as the experiments exceeded our time limit.}\label{fig:throughput}
\end{figure} %

\begin{figure}[]
\centering
  \begin{minipage}[t]{0.49\textwidth}
    \includegraphics[width=\columnwidth]{plot/Adv-5D-Uniform-10M.pdf}
  \end{minipage} %
  \begin{minipage}[t]{0.49\textwidth}
    \includegraphics[width=\columnwidth]{plot/Adv-3D-Cosmo-298M.pdf}
  \end{minipage} %
  \caption{Plot of running time (in seconds) vs.\ insertion batch size for the dynamic and static methods using 48 cores with hyper-threading on 5D-Uniform-10M and 3D-Cosmo-298M. The plot is in log-log scale.}\label{fig:advantage}
\end{figure} %

\begin{figure}[]
\centering
  \begin{minipage}[t]{0.49\textwidth}
    \includegraphics[width=\columnwidth]{plot/AdvDel-5D-Uniform-10M.pdf}
  \end{minipage} %
  \begin{minipage}[t]{0.49\textwidth}
    \includegraphics[width=\columnwidth]{plot/AdvDel-3D-Cosmo-298M.pdf}
  \end{minipage} %
  \caption{Plot of running time (in seconds) vs.\ deletion batch size for the dynamic and static methods using 48 cores with hyper-threading on 5D-Uniform-10M and 3D-Cosmo-298M. The plot is in log-log scale.}\label{fig:advantage-deletion}
% \caption{Parallel performance of the batch-dynamic algorithm on varying batch sizes.}
\end{figure}

